Sharp phase transition for Cox percolation

We prove the sharpness of the percolation phase transition for a class of Cox percolation models, i.e., models of continuum percolation in a random environment. The key requirements are that the environment has a finite range of dependence and satisfies a local boundedness condition, however the FKG inequality need not hold. The proof combines the OSSS inequality with a coarse-graining construction.

==> comp.tex <==

%COMP PERC
\subsection{Comparison of pivotal probabilities -- Proof of Proposition \ref{ess_lem}}
	In order to compare the pivotal probabilities with respect to the Delaunay vertices to the pivotal probabilities with respect to the planar devices, we will rely on the Aizenman--Grimmett method of essential enhancements \cite{strictGrim}. While originally stated for lattice percolation problems, it has been successfully extended to the continuum setting in \cite{strictIneq}. The key idea is to transform a configuration with Delaunay-pivotal point into a configuration with a pivotal planar device at a bounded probabilistic cost. To achieve this goal, we adapt the geometric construction from \cite[Lemma 3.2]{strictIneq}.

	%DEF Y
	To make this precise, let $E_{\Del, r}(x)$ be the event that $x \in B_r$ is Delaunay pivotal in the sense that $f_r(\Xp, \Xs, \Xd \cup\{x\}) \ne f_r(\Xp, \Xs, \Xd)$. Similarly, we let $E_{\ms p, r}(x)$ denote the event that a planar device placed at $x$ is pivotal. In order to transition from $E_{\Del, r}(x)$ to $E_{\ms p, r}(x)$, we leave $\Xp \sm B_{r_0}(x)$, $\Xs \sm B_{r_0}(x)$ and $\Xd$ unchanged, and only modify $\Xp$ and $\Xs$ within $B_{r_0}(x)$, where $r_0 := \rstab + 8$. First, based on the network constructed from $\Xd$ and $\Xps \sm B_{r_0}(x)$, 	we let $T$ and $V$ denote the points that are connected to $\pa B_r$ and to $\pa B_2$, respectively. Now, we start to sequentially generate the remaining points in $\Xps \cap B_{r_0}(x)$ in a decreasing radial distance from $x$. We continue this generation of points until one of the new points $y$ connects to $T$ or to $V$. We may assume that it connects to $V$, and then write $s := |x - y|$ for its distance to $x$. 

	%DEF Z
Now, we let $F$ denote the event that $B_{s + 0.05}(x)$ contains some vertex from $T$, and let $z$ be such a vertex. If the event $F$ does not occur, then we continue exploring radially towards $x$ until we find a vertex $z$ that connects to $T$. Now, we let $G$ be the event that (i) $V \cap T = \es$ and (ii) both $y$ and $z$ exist. Then, we observe that the event $G$ always occurs under the event $E_{\Del, r}(x)$. Hence, we only rely on the pivotal event $E_{\Del, r}(x)$ to ensure that the event $G$ occurs and from now on work under $G$. It remains to show that the conditional probability that a planar device at $x$ is pivotal is bounded away from 0. 


To achieve this goal, we distinguish between the cases $G \cap F$ and $G \sm F$. Since in the case $G \sm F$ the adaptation from the construction of \cite[Lemma 3.2]{strictIneq} proceeds along similar lines, we concentrate on $G \cap F$ henceforth. In the case $G \cap F$, we build on the steps from \cite[Lemma 3.2]{strictIneq} in order to construct target locations $a_1, \dots, a_M, b_1, \dots, b_M \in B_s(x)$ with $M:= \lfloor 2 \rstab \rfloor + 16$ such that the following items are satisfied:
\beit
\im $\lvert a_i - a_{i-1}\rvert \le0.9$ and $\lvert b_i - b_{i - 1}\rvert  \le 0.9$ for $1 \le i \le M$ (with $a_0 := y$, $b_0 :=z$);
\im $\lvert a_M - x\rvert  \le 0.9$ and $\lvert a_i - x\rvert >1.1$ for $i\le M - 1$;
\im $\lvert b_M - x\rvert  \le 0.9$ and $\lvert b_i - x\rvert >1.1$ for $i\le M - 1$;
\im $\lvert a_i - b_i\rvert  > 1.02$;
\enit
Then, we let $H$ denote the event that (i) there is a point from $\Xp$ at distance at most $0.05$ from each of the target locations, and (ii) there are no other points in $B_s(x)$. In particular, under the event $H$, a planar device placed at position $x$ is pivotal. Since the probability of the event $H$ is bounded away from 0 regardless of the values of $x$ or $r$, we conclude the proof in the case $G \cap F$. 


==> rev.tex <==


 %
 %REV BOUND
 %
 \subsection{The exploration CTDT -- Proof of Lemma \ref{rev_lem}}

 %
 %CONSTR
 %

 To prove Lemma \ref{rev_lem}, we loosely proceed along the lines of \cite[Theorem 8.2]{lpy}. We first explain how to define the CTDT $Z = Z(r)$. For each $s \le r$ we construct a stopping set $Z(r, s)$ determining $\{B_1 \lrsa \partial B_r\}$ as follows. Since the Delaunay triangulation is constructed on the superposition of a Poisson point process with a fixed grid, the model has a finite deterministic radius of stabilization $\rstab < \ff$. This means that whether a point $x \in \R^2$ belongs to $\SS(\Xd)$ only depends on the configuration  of points from $\Xd$ that are at distance at most $\rstab$ from $x$. Now, let 
$X(s, r) \su \Xps \cap B_r$ denote the family of all $X_i \in \Xps$ that are contained in a connected component intersecting the shell $\pa B_s$. We then set 
$$Z(r, s) := (X(s, r) \cup \pa B_s) \oplus B_{\rstab}.$$
Finally, we consider the randomization $Z(r) := Z(r,U)$, where $U$ is uniform at random in $(0, r)$.

After having constructed $Z(r)$ two steps are remaining to complete the proof of Lemma \ref{rev_lem}. First, Section \ref{rev_sec} derives the asserted revealment probabilities. Second, Section \ref{osss_sec} shows that the randomized CTDT satisfies the conditions of the continuous OSSS inequality from \cite[Theorem 4.2]{lpy}.

  %
 %REV BOUND
 %
 \subsubsection{Bound on revealment probabilities}
 \label{rev_sec}
 In the proof of \cite[Theorem 8.2]{lpy}, to bound the revealment probability $\P(x \in Z(r, s))$, the FKG inequality is used, which is not available in the Cox percolation model. Hence, in the present situation, we provide an new solution relying on an alternative definition of the finite-volume percolation probabilities $\th_r(\la)$, $r > 0$. Instead of defining percolation as having a connection to $\pa B_r$ from the origin $o$, we only demand that there is a connection to $\pa B_2$. 

More precisely, after covering $\pa B_{\rstab}(x)$ by a constant number of radius-2 disks centered at $\pa B_{\rstab}(x)$, we deduce that
\begin{align*}
	\P(x \in Z(r, s)) &\le \P\big(B_{\rstab}(x) \lrsa \pa B_s\big)	\le c' \th_{|s - |x|| - \rstab},
\end{align*}
where we set $\th_a = 1$ for $a \le 0$. Hence, when averaging over $s \in [0, r]$, we obtain that
\begin{align*}
	\P(x \in Z(r)) &\le c'r^{-1}\int_0^r \th_{|s - |x|| - \rstab}\d s
	\le c'r^{-1}  \int_0^{r - \rstab} \th_t\d t
	\le c'r^{-1}\int_0^r \th_t \d t.
\end{align*}




 %
 %COND SEC
 %
 \subsubsection{Verification of OSSS conditions}
 \label{osss_sec}
 To conclude the proof of Lemma \ref{rev_lem}, we need to verify that $Z(r, s)$ is a CTDT satisfying the conditions of \cite[Theorem 4.2]{lpy}. To that end, we may proceed along the lines of \cite[Theorem 8.2]{lpy} without major changes. Nevertheless, to make the manuscript self-contained, we include a broad overview, referring to \cite{lpy} for the full details. 

 To represent $Z(r, s)$ as CTDT, we first describe auxiliary random sets $\{S_i\}_{i \ge 0}$ and $\{E_i\}_{i \ge 0}$ inductively as follows, starting with $E_0 := \partial B_s$, $E_1 := \partial B_s \oplus B_{\rstab}$, $S_0 := \es$ and $S_1\su \Xps$ as the union of all components based on points in $E_1$ and intersecting $\partial B_s$.  Suppose now that $(S_0, E_0), \dots, (S_m, E_m)$ are already constructed. The algorithm terminates if $S_m = S_{m - 1}$, and we set $E_\ff := E_m$. Otherwise, we set $E_{m + 1} := (S_m \cup E_0) \oplus B_{\rstab}$ and $S_{m + 1}$ as the union of $S_m$ and all points in $\Xps$ that are at distance at most 1 from an element of $S_m$. 

%DEF Z_r
 With these auxiliary sets, we now define $Z(r, s)_t$, $t \ge 0$ as follows. For a non-negative integer $m$ and $t \in [m, m + 1)$, we set $Z(r, s)_t := Z(r, s)_{m-} \cup (S_{m + 1} \oplus B_{(t - m)\rstab})$. Then,  $\bigcup_{t \ge 0}Z(r, s)_t = Z(r, s)$, and we now discuss the conditions of \cite[Theorem 4.2]{lpy}.
 \beit
 \im[]{\bf Stopping-set property.} Since $\rstab$ is a radius of stabilization, we deduce that modifying either of the point processes $\Xp$, $\Xs$ or $\Xd$ outside $Z(r, s)_t$ does not change $Z(r, s)_t$. 
 \im[]{\bf CTDT.} The sets $Z(r, s)_t$ are increasing in $t$. Moreover, we have $\bigcap_{u > 0} B_{u \rstab}(o) = o$. Hence, the CTDT property holds. 
 \im[]{\bf Determination property.} Since every percolating component must cross $\pa B_s$, we conclude that the value of $f$ is already determined by the configuration of $\Xp$, $\Xs$ and $\Xd$ inside $Z(r, s)$.
 \im[]{\bf Zero-set property.} Since $|\pa B_u(o)| = 0$ for every $u > 0$, we deduce that $Z(r, s)_t \sm Z(r, s)_{t-}$ is a zero set for every $t > 0$.
 \enit


